Practicable Simulation-Free Model Order Reduction by Nonlinear Moment Matching

In this paper, a practicable simulation-free model order reduction method by nonlinear moment matching is developed. Based on the steady-state interpretation of linear moment matching, we comprehensively explain the extension of this reduction concept to nonlinear systems presented in [1], provide some new insights and propose some simplifications to achieve a feasible and numerically efficient nonlinear model reduction algorithm. This algorithm relies on the solution of nonlinear systems of equations rather than on the expensive simulation of the original model or the difficult solution of a nonlinear partial differential equation.

==> auxfiles/algos.tex <==
\begin{algorithm}
	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	\SetKwFor{Foreach}{for each}{do}{endfor}
	\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{endif}
	\Input{A method \emph{m}}
	\Output{result}
	\Foreach { $x \in M_{x}$}{
		do something
	}
	\caption{Algorithm}\label{Method}
\end{algorithm}



==> auxfiles/formulas.tex <==
\begin{subequations}
\begin{align}
\boldsymbol{E} \, \dot{\boldsymbol{x}}(t) &= \boldsymbol{A} \, \boldsymbol{x}(t) + \boldsymbol{B} \, \boldsymbol{u}(t), \\
\boldsymbol{y}(t) &= \boldsymbol{C} \, \boldsymbol{x}(t)
\end{align}
\end{subequations}

\begin{subequations}
	\begin{align}
	\overbrace{\boldsymbol{W}^{\mathsf{T}} \, \boldsymbol{E} \, \boldsymbol{V}}^{\boldsymbol{E}_{\mathrm{r}}} \, \dot{\boldsymbol{x}}_{\mathrm{r}}(t) &= \overbrace{\boldsymbol{W}^{\mathsf{T}} \, \boldsymbol{A} \, \boldsymbol{V}}^{\boldsymbol{A}_{\mathrm{r}}} \, \boldsymbol{x}_{\mathrm{r}}(t) + \overbrace{\boldsymbol{W}^{\mathsf{T}} \, \boldsymbol{B}}^{\boldsymbol{B}_{\mathrm{r}}} \, \boldsymbol{u}(t), \\
	\boldsymbol{y}_{\mathrm{r}}(t) &= \underbrace{\boldsymbol{C} \, \boldsymbol{V}}_{\boldsymbol{C}_{\mathrm{r}}} \, \boldsymbol{x}_{\mathrm{r}}(t),
	\end{align}
\end{subequations}

\begin{subequations}
	\begin{align}
	\boldsymbol{E}_{\mathrm{r}} \, \dot{\boldsymbol{x}}_{\mathrm{r}}(t) &= \boldsymbol{A}_{\mathrm{r}} \, \boldsymbol{x}_{\mathrm{r}}(t) + \boldsymbol{B}_{\mathrm{r}} \, \boldsymbol{u}(t), \\ 
	\boldsymbol{y}_{\mathrm{r}}(t) &= \boldsymbol{C}_{\mathrm{r}} \, \boldsymbol{x}_{\mathrm{r}}(t),
	\end{align}
\end{subequations}

\begin{equation}
\resizebox{0.89\linewidth}{!}{
	$\mathrm{Ran}(\boldsymbol{V}) \in \mathrm{span}\left\{
	(\sigma_1 \boldsymbol{E} \!-\! \boldsymbol{A})^{-1} \! \boldsymbol{B} \, \boldsymbol{r}_1, \ldots, (\sigma_r \boldsymbol{E} \!-\! \boldsymbol{A})^{-1} \! \boldsymbol{B} \, \boldsymbol{r}_r\right\}$}
\end{equation}

\begin{equation}
\resizebox{0.89\linewidth}{!}{
	$\mathrm{Ran}(\boldsymbol{W}) \in \mathrm{span}\left\{
	(\mu_1 \boldsymbol{E} \!-\! \boldsymbol{A})^{- \! \mathsf T}\boldsymbol{C}^{\mathsf T} \boldsymbol{l}_1, \ldots, (\mu_r \boldsymbol{E} \!-\! \boldsymbol{A})^{- \! \mathsf T}\boldsymbol{C}^{\mathsf T} \boldsymbol{l}_r\right\}$}
\end{equation}

%relies on choosing the projection matrices $\boldsymbol{V}$ and $\boldsymbol{W}$ as bases of rational Krylov subspaces.

\begin{equation}
\frac{\mathrm{d}^{i} \boldsymbol{G}(s)}{\mathrm{d}s^{i}}
\end{equation}

%In fact, it can be shown [32] that the resulting reduced
%order model interpolates the original transfer function
%𝐺(𝑠) and its derivatives at the approximation frequencies
%𝜎 and 𝜇, also called shifts or expansion points.
%
%then the reduced order model is guaranteed to match 2n
%moments of the FOM, that is Taylor series coefficients about
% 2C [4]. Note that an analogous result applies to the case
%where  is not a scalar value but a set of complex frequencies
% = figq
%i=1 with associated dimensions of the respective
%Krylov subspaces fnigq
%i=1 where
%Pq
%i=1 ni=n. In this case,
%known as multipoint Pad´e, the projection subspace is given
%by the union of all individual rational Krylov subspaces. In
%the following we will make no distinction in the notation for
%the sake of simplicity.

%=========================== Sylvester
$\boldsymbol{S}_v \in \mathbb{C}^{r \times r}$, $\boldsymbol{R} \in \mathbb{C}^{m \times r}$, observable pair $(\boldsymbol{R}, \boldsymbol{S}_v)$

$\boldsymbol{S}_w \in \mathbb{C}^{r \times r}$, $\boldsymbol{L} \in \mathbb{C}^{p \times r}$, controllable pair $(\boldsymbol{S}_w, \boldsymbol{L})$

$\boldsymbol{S}_w := \mathrm{diag}(\mu_1, \ldots, \mu_r) \in \mathbb{C}^{r \times r}$

$\boldsymbol{L} := \left[\boldsymbol{l}_1, \ldots, \boldsymbol{l}_r \right] \in \mathbb{C}^{p \times r}$

\footnote{For SISO ($m\!=\!1, p\!=\!1$) replace $\boldsymbol{B} \in \mathbb{R}^{n \times m} \to \boldsymbol{b} \in \mathbb{R}^{n}$ and $\boldsymbol{C} \in \mathbb{R}^{p \times n} \to \boldsymbol{c}^{\mathsf T} \in \mathbb{R}^{1 \times n}$.}

$\boldsymbol{x}_{\mathrm{r}}(t) = \mathrm{e}^{\boldsymbol{S}_v t} \, \boldsymbol{x}_{\mathrm{r},0}$

%=======================================================================
%====================== Section III

%In many applications, the classical Petrov-Galerkin projection with linear mappings given by the matrices $\boldsymbol{V}, \boldsymbol{W}$ is applied to the nonlinear system \eqref{eq:nonlinear-FOM} 


$\boldsymbol{x}(t) = \boldsymbol{\nu}(\boldsymbol{x}_{\mathrm{r}}(t))$, 

smooth mapping $\boldsymbol{\nu}(\boldsymbol{x}_{\mathrm{r}}) : \mathbb{R}^r \to \mathbb{R}^n$, 

$\boldsymbol{x} = \boldsymbol{\nu}(\boldsymbol{x}_{\mathrm{r}}) \ \widehat{=} \ \boldsymbol{V} \, \boldsymbol{x}_{\mathrm{r}}$,

$\boldsymbol{V} \ \widehat{=} \ \frac{\partial \boldsymbol{\nu}(\boldsymbol{x}_{\mathrm{r}})}{\partial \boldsymbol{x}_{\mathrm{r}}}$
\\\\
$\boldsymbol{x}_{\mathrm{r}}(t) = \boldsymbol{\omega}(\boldsymbol{x}(t))$, 

smooth mapping $\boldsymbol{\omega}(\boldsymbol{x}) : \mathbb{R}^n \to \mathbb{R}^r$, 

$\boldsymbol{x}_{\mathrm{r}} = \boldsymbol{\omega}(\boldsymbol{x}) \ \widehat{=} \ \boldsymbol{W}^{\mathsf T} \, \boldsymbol{x}$

$\boldsymbol{W}^{\mathsf T} \ \widehat{=} \ \frac{\partial \boldsymbol{\omega}(\boldsymbol{x})}{\partial \boldsymbol{x}}$,
\\\\
$\boldsymbol{\omega}(\boldsymbol{\nu}(\boldsymbol{x}_{\mathrm{r}})) = \boldsymbol{x}_{\mathrm{r}}$ corresponds to $\boldsymbol{W}^{\mathsf T} \boldsymbol{V} \boldsymbol{x}_{\mathrm{r}} = \boldsymbol{x}_{\mathrm{r}}$ which implies $\boldsymbol{W}^{\mathsf T} \boldsymbol{V} = \boldsymbol{I}_r$

projector is given by the mapping $\varrho : \mathbb{R}^n \to \mathbb{R}^n$ and corresponds to the projector $\boldsymbol{P} = \boldsymbol{V}(\boldsymbol{W}^{\mathsf T} \boldsymbol{V})^{-1} \boldsymbol{W}^{\mathsf T}$

==> tikz/lin-sys-lin-SG_steady-state.tex <==
\begin{tikzpicture}

  % Knoten / Blöcke
  \UeFunk[align = left, inner sep = 6 pt]{linSigGen}{-0.9, 0}{0.6 cm}{
		$\begin{aligned}
		\dot{\boldsymbol{x}}_{\mathrm{r}}(t) &= \boldsymbol{S}_{v} \, \boldsymbol{x}_{\mathrm{r}}(t) \\[0.2em]
		\boldsymbol{u}(t) &= \boldsymbol{R} \, \boldsymbol{x}_{\mathrm{r}}(t)
		\end{aligned}$
  }
  \UeFunk[align = left, inner sep = 6 pt]{FOM}{6.3, 0}{0.6 cm}{
	    $\begin{aligned}
	    \boldsymbol{E} \, \dot{\boldsymbol{x}}(t) &= \boldsymbol{A} \, \boldsymbol{x}(t) + \boldsymbol{B} \, \boldsymbol{u}(t) \\[0.2em]
	    \boldsymbol{y}(t) &= \boldsymbol{C} \, \boldsymbol{x}(t) 
	    \end{aligned}$
  } 
  \UeFunk[align = left, inner sep = 6 pt]{ROM}{6.3, -4}{0.6 cm}{
	  	$\begin{aligned}
     	\boldsymbol{W}^{\mathsf T} \boldsymbol{E} \boldsymbol{V} \, \dot{\boldsymbol{x}}_{\mathrm{r}}(t) &= \boldsymbol{W}^{\mathsf T} \boldsymbol{A} \boldsymbol{V} \, \boldsymbol{x}_{\mathrm{r}}(t) + \boldsymbol{W}^{\mathsf T} \boldsymbol{B} \, \boldsymbol{u}(t) \\[0.2em]
     	\boldsymbol{y}_{\mathrm{r}}(t) &= \boldsymbol{C} \boldsymbol{V} \, \boldsymbol{x}_{\mathrm{r}}(t)
     	\end{aligned}$
  }
  
  \Verzweigung{verzw-u}{2, 0}{3 pt}
  
  \Summationsstelle{summation}{11.1, 0}{0.4 cm}

   
  % Signalflüsse
  \draw[thick, -latex'] (linSigGen) -- (FOM) node[pos = 0.49, above] {$\boldsymbol{u}(t) = \boldsymbol{R} \, \mathrm{e}^{\boldsymbol{S}_v t} \, \boldsymbol{x}_{\mathrm{r},0}$};
  \draw[thick, -latex'] (verzw-u) |- (ROM);
  \draw[thick, -latex'] (FOM.east) -- (summation) node[pos = 0.51, above] {$\boldsymbol{y}(t)$};
  \draw[thick, -latex'] (ROM.east) -| (summation) node[pos = 0.28, above] {$\boldsymbol{y}_{\mathrm{r}}(t)$};
  \draw[thick, -latex'] (summation) -- (12.9, 0) node[pos = 0.49, above] {$\boldsymbol{e}(t)=\boldsymbol{0}$};
  
  \draw[thick, -latex'] (linSigGen) -- + (0,1.7) node[pos = 0.7, right] {$\boldsymbol{x}_{\mathrm{r},0}$} -- (linSigGen);
%  \draw[thick, -latex'] (linSigGen) -- + (0,1.7) node[pos = 0.7, right] {$\boldsymbol{x}_{\mathrm{r},0} = \boldsymbol{V}^{\mathsf T} \boldsymbol{x}_{0}$} -- (linSigGen);
  \draw[thick, -latex'] (FOM) -- + (0,1.7) node[pos = 0.7, right] {$\boldsymbol{x}_{0} = \boldsymbol{V} \boldsymbol{x}_{\mathrm{r},0}$} -- (FOM);
  \draw[thick, -latex'] (ROM) -- + (0,1.7) node[pos = 0.7, right] {$\boldsymbol{x}_{\mathrm{r},0} = \boldsymbol{W}^{\mathsf T} \boldsymbol{x}_{0}$} -- (ROM);

  % Beschriftungen
  \node[outer sep = 0.1 cm, below] at (linSigGen.south) {\text{linear signal generator}};
  \node[outer sep = 0.1 cm, below] at (FOM.south) {\text{FOM}};
  \node[outer sep = 0.1 cm, below] at (ROM.south) {\text{ROM}};
  
  \node[outer sep = 0.3 cm, below] at (summation.west) {$-\ $};
  
\end{tikzpicture}

==> tikz/nonlin-sys-nonlin-SG_steady-state.tex <==
\begin{tikzpicture}

  % Knoten / Blöcke
  \UeFunk[align = left, inner sep = 6 pt]{nonlinSigGen}{0, 0}{0.6 cm}{
		$\begin{aligned}
		\dot{\boldsymbol{x}}_{\mathrm{r}}(t) &= \boldsymbol{s}_{v}\big(\boldsymbol{x}_{\mathrm{r}}(t)\big) \\[0.2em]
		\boldsymbol{u}(t) &= \boldsymbol{r}\big(\boldsymbol{x}_{\mathrm{r}}(t)\big)
		\end{aligned}$
  }
  \UeFunk[align = left, inner sep = 6 pt]{FOM}{6.7, 0}{0.6 cm}{
	    $\begin{aligned}
	    \dot{\boldsymbol{x}}(t) &= \boldsymbol{f}\big(\boldsymbol{x}(t), \boldsymbol{u}(t)\big) \\[0.2em]
	    \boldsymbol{y}(t) &= \boldsymbol{h}\big(\boldsymbol{x}(t)\big)
	    \end{aligned}$
  } 
  \UeFunk[align = left, inner sep = 6 pt]{ROM}{6.7, -4}{0.6 cm}{
	  	$\begin{aligned}
     	\dot{\boldsymbol{x}}_{\mathrm{r}}(t) &= \left.\frac{\partial \boldsymbol{\omega}(\boldsymbol{x})}{\partial \boldsymbol{x}}\right|_{\boldsymbol{x}=\boldsymbol{\nu}(\boldsymbol{x}_{\mathrm{r}})} \, \boldsymbol{f}\big(\boldsymbol{\nu}(\boldsymbol{x}_{\mathrm{r}}(t)), \boldsymbol{u}(t)\big) \\[0.2em]
     	\boldsymbol{y}_{\mathrm{r}}(t) &= \boldsymbol{h}\big(\boldsymbol{\nu}(\boldsymbol{x}_{\mathrm{r}}(t))\big)
     	\end{aligned}$
  }
  
  \Verzweigung{verzw-u}{2.5, 0}{3 pt}
  
  \Summationsstelle{summation}{11.5, 0}{0.4 cm}

   
  % Signalflüsse
  \draw[thick, -latex'] (nonlinSigGen) -- (FOM) node[pos = 0.49, above] {$\boldsymbol{u}(t)$};
  \draw[thick, -latex'] (verzw-u) |- (ROM);
  \draw[thick, -latex'] (FOM.east) -- (summation) node[pos = 0.76, above] {$\boldsymbol{y}(t)$};
  \draw[thick, -latex'] (ROM.east) -| (summation) node[pos = 0.25, above] {$\boldsymbol{y}_{\mathrm{r}}(t)$};
  \draw[thick, -latex'] (summation) -- (13.5, 0) node[pos = 0.49, above] {$\boldsymbol{e}(t)=\boldsymbol{0}$};
  
  \draw[thick, -latex'] (nonlinSigGen) -- + (0,1.7) node[pos = 0.7, right] {$\boldsymbol{x}_{\mathrm{r},0}$} -- (nonlinSigGen);
%  \draw[thick, -latex'] (nonlinSigGen) -- + (0,1.7) node[pos = 0.7, right] {$\boldsymbol{x}_{\mathrm{r},0} = \boldsymbol{\omega}(\boldsymbol{x}_{0})$} -- (nonlinSigGen);
  \draw[thick, -latex'] (FOM) -- + (0,1.7) node[pos = 0.7, right] {$\boldsymbol{x}_{0} = \boldsymbol{\nu}(\boldsymbol{x}_{\mathrm{r},0})$} -- (FOM);
  \draw[thick, -latex'] (ROM) -- + (0,1.7) node[pos = 0.7, right] {$\boldsymbol{x}_{\mathrm{r},0} = \boldsymbol{\omega}(\boldsymbol{x}_{0})$} -- (ROM);

  % Beschriftungen
  \node[outer sep = 0.1 cm, below] at (nonlinSigGen.south) {\text{nonlinear signal generator}};
  \node[outer sep = 0.1 cm, below] at (FOM.south) {\text{FOM}};
  \node[outer sep = 0.1 cm, below] at (ROM.south) {\text{ROM}};
  
  \node[outer sep = 0.3 cm, below] at (summation.west) {$-\ $};
  
\end{tikzpicture}
